Neurosymbolic Grounding for Compositional World Models

We introduce Cosmos, a framework for object-centric world modeling that is designed for compositional generalization (CompGen), i.e., high performance on unseen input scenes obtained through the composition of known visual "atoms." The central insight behind Cosmos is the use of a novel form of neurosymbolic grounding. Specifically, the framework introduces two new tools: (i) neurosymbolic scene encodings, which represent each entity in a scene using a real vector computed using a neural encoder, as well as a vector of composable symbols describing attributes of the entity, and (ii) a neurosymbolic attention mechanism that binds these entities to learned rules of interaction. Cosmos is end-to-end differentiable; also, unlike traditional neurosymbolic methods that require representations to be manually mapped to symbols, it computes an entity's symbolic attributes using vision-language foundation models. Through an evaluation that considers two different forms of CompGen on an established blocks-pushing domain, we show that the framework establishes a new state-of-the-art for CompGen in world modeling. Artifacts are available at: https://trishullab.github.io/cosmos-web/

==> sections/fig-schematic.tex <==
\begin{figure}
    \begin{minipage}{\linewidth}
        \centering
        {\includegraphics[width=\linewidth]{imgs/fig-schematic-theirs.pdf}}
    \end{minipage}
    \hbox to \linewidth{\leaders\hbox to 2pt{\hss . \hss}\hfil} \\
    \begin{minipage}{\textwidth}
        \centering
        {\includegraphics[width=\linewidth]{imgs/fig-schematic-ours.pdf}}
    \end{minipage}
    
    \caption{Overview of world modeling (top) vs symbolically grounded world modeling (bottom). }
    \label{fig:schematic}
\end{figure}

